Towards Rational Consensus in Honest Majority

Distributed consensus protocols reach agreement among $n$ players in the presence of $f$ adversaries; different protocols support different values of $f$. Existing works study this problem for different adversary types (captured by threat models). There are three primary threat models: (i) Crash fault tolerance (CFT), (ii) Byzantine fault tolerance (BFT), and (iii) Rational fault tolerance (RFT), each more general than the previous. Agreement in repeated rounds on both (1) the proposed value in each round and (2) the ordering among agreed-upon values across multiple rounds is called Atomic BroadCast (ABC). ABC is more generalized than consensus and is employed in blockchains. This work studies ABC under the RFT threat model. We consider $t$ byzantine and $k$ rational adversaries among $n$ players. We also study different types of rational players based on their utility towards (1) liveness attack, (2) censorship or (3) disagreement (forking attack). We study the problem of ABC under this general threat model in partially-synchronous networks. We show (1) ABC is impossible for $n/3< (t+k) <n/2$ if rational players prefer liveness or censorship attacks and (2) the consensus protocol proposed by Ranchal-Pedrosa and Gramoli cannot be generalized to solve ABC due to insecure Nash equilibrium (resulting in disagreement). For ABC in partially synchronous network settings, we propose a novel protocol \textsf{pRFT}(practical Rational Fault Tolerance). We show \textsf{pRFT} achieves ABC if (a) rational players prefer only disagreement attacks and (b) $t < \frac{n}{4}$ and $(t + k) < \frac{n}{2}$. In \textsf{pRFT}, we incorporate accountability (capturing deviating players) within the protocol by leveraging honest players. We also show that the message complexity of \textsf{pRFT} is at par with the best consensus protocols that guarantee accountability.

==> ref.tex <==
%%% -*-BibTeX-*-
%%% Do NOT edit. File created by BibTeX with style
%%% ACM-Reference-Format-Journals [18-Jan-2012].

\begin{thebibliography}{47}

%%% ====================================================================
%%% NOTE TO THE USER: you can override these defaults by providing
%%% customized versions of any of these macros before the \bibliography
%%% command.  Each of them MUST provide its own final punctuation,
%%% except for \shownote{}, \showDOI{}, and \showURL{}.  The latter two
%%% do not use final punctuation, in order to avoid confusing it with
%%% the Web address.
%%%
%%% To suppress output of a particular field, define its macro to expand
%%% to an empty string, or better, \unskip, like this:
%%%
%%% \newcommand{\showDOI}[1]{\unskip}   % LaTeX syntax
%%%
%%% \def \showDOI #1{\unskip}           % plain TeX syntax
%%%
%%% ====================================================================

\ifx \showCODEN    \undefined \def \showCODEN     #1{\unskip}     \fi
\ifx \showDOI      \undefined \def \showDOI       #1{#1}\fi
\ifx \showISBNx    \undefined \def \showISBNx     #1{\unskip}     \fi
\ifx \showISBNxiii \undefined \def \showISBNxiii  #1{\unskip}     \fi
\ifx \showISSN     \undefined \def \showISSN      #1{\unskip}     \fi
\ifx \showLCCN     \undefined \def \showLCCN      #1{\unskip}     \fi
\ifx \shownote     \undefined \def \shownote      #1{#1}          \fi
\ifx \showarticletitle \undefined \def \showarticletitle #1{#1}   \fi
\ifx \showURL      \undefined \def \showURL       {\relax}        \fi
% The following commands are used for tagged output and should be
% invisible to TeX
\providecommand\bibfield[2]{#2}
\providecommand\bibinfo[2]{#2}
\providecommand\natexlab[1]{#1}
\providecommand\showeprint[2][]{arXiv:#2}

\bibitem[Abraham et~al\mbox{.}(2019)]%
        {Abraham2019AsyncCheapTalks}
\bibfield{author}{\bibinfo{person}{Ittai Abraham}, \bibinfo{person}{Danny Dolev}, \bibinfo{person}{Ivan Geffner}, {and} \bibinfo{person}{Joseph~Y. Halpern}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Implementing Mediators with Asynchronous Cheap Talk}. In \bibinfo{booktitle}{\emph{Proceedings of the 2019 ACM Symposium on Principles of Distributed Computing}} (Toronto ON, Canada) \emph{(\bibinfo{series}{PODC '19})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{501–510}.
\newblock
\showISBNx{9781450362177}
\urldef\tempurl%
\url{https://doi.org/10.1145/3293611.3331623}
\showDOI{\tempurl}


\bibitem[Abraham et~al\mbox{.}(2006)]%
        {Abraham2006RationalMPC}
\bibfield{author}{\bibinfo{person}{Ittai Abraham}, \bibinfo{person}{Danny Dolev}, \bibinfo{person}{Rica Gonen}, {and} \bibinfo{person}{Joe Halpern}.} \bibinfo{year}{2006}\natexlab{}.
\newblock \showarticletitle{Distributed Computing Meets Game Theory: Robust Mechanisms for Rational Secret Sharing and Multiparty Computation}. In \bibinfo{booktitle}{\emph{Proceedings of the Twenty-Fifth Annual ACM Symposium on Principles of Distributed Computing}} (Denver, Colorado, USA) \emph{(\bibinfo{series}{PODC '06})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{53–62}.
\newblock
\showISBNx{1595933840}
\urldef\tempurl%
\url{https://doi.org/10.1145/1146381.1146393}
\showDOI{\tempurl}


\bibitem[Abraham et~al\mbox{.}(2020)]%
        {Abraham2020SyncHotstuff}
\bibfield{author}{\bibinfo{person}{Ittai Abraham}, \bibinfo{person}{Dahlia Malkhi}, \bibinfo{person}{Kartik Nayak}, \bibinfo{person}{Ling Ren}, {and} \bibinfo{person}{Maofan Yin}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{Sync HotStuff: Simple and Practical Synchronous State Machine Replication}. In \bibinfo{booktitle}{\emph{2020 IEEE Symposium on Security and Privacy (SP)}}. \bibinfo{pages}{106--118}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/SP40000.2020.00044}
\showDOI{\tempurl}


\bibitem[Aiyer et~al\mbox{.}(2005)]%
        {Aiyer2005BAR}
\bibfield{author}{\bibinfo{person}{Amitanand~S. Aiyer}, \bibinfo{person}{Lorenzo Alvisi}, \bibinfo{person}{Allen Clement}, \bibinfo{person}{Mike Dahlin}, \bibinfo{person}{Jean-Philippe Martin}, {and} \bibinfo{person}{Carl Porth}.} \bibinfo{year}{2005}\natexlab{}.
\newblock \showarticletitle{BAR Fault Tolerance for Cooperative Services}.
\newblock \bibinfo{journal}{\emph{SIGOPS Oper. Syst. Rev.}} \bibinfo{volume}{39}, \bibinfo{number}{5} (\bibinfo{date}{oct} \bibinfo{year}{2005}), \bibinfo{pages}{45–58}.
\newblock
\showISSN{0163-5980}
\urldef\tempurl%
\url{https://doi.org/10.1145/1095809.1095816}
\showDOI{\tempurl}


\bibitem[Amoussou-Guenou et~al\mbox{.}(2020)]%
        {Amoussou2020AAMASRCEquilibrium}
\bibfield{author}{\bibinfo{person}{Yackolley Amoussou-Guenou}, \bibinfo{person}{Bruno Biais}, \bibinfo{person}{Maria Potop-Butucaru}, {and} \bibinfo{person}{Sara Tucci-Piergiovanni}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{Rational vs Byzantine Players in Consensus-Based Blockchains}. In \bibinfo{booktitle}{\emph{Proceedings of the 19th International Conference on Autonomous Agents and MultiAgent Systems}} (Auckland, New Zealand) \emph{(\bibinfo{series}{AAMAS '20})}. \bibinfo{publisher}{International Foundation for Autonomous Agents and Multiagent Systems}, \bibinfo{address}{Richland, SC}, \bibinfo{pages}{43–51}.
\newblock
\showISBNx{9781450375184}


\bibitem[Asharov et~al\mbox{.}(2011)]%
        {Asharov2011RationalCrypto}
\bibfield{author}{\bibinfo{person}{Gilad Asharov}, \bibinfo{person}{Ran Canetti}, {and} \bibinfo{person}{Carmit Hazay}.} \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{Towards a Game Theoretic View of Secure Computation}. In \bibinfo{booktitle}{\emph{Advances in Cryptology -- EUROCRYPT 2011}}, \bibfield{editor}{\bibinfo{person}{Kenneth~G. Paterson}} (Ed.). \bibinfo{publisher}{Springer Berlin Heidelberg}, \bibinfo{address}{Berlin, Heidelberg}, \bibinfo{pages}{426--445}.
\newblock
\showISBNx{978-3-642-20465-4}


\bibitem[Aublin et~al\mbox{.}(2013)]%
        {Aublin2013RBFT}
\bibfield{author}{\bibinfo{person}{Pierre-Louis Aublin}, \bibinfo{person}{Sonia~Ben Mokhtar}, {and} \bibinfo{person}{Vivien Quéma}.} \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{RBFT: Redundant Byzantine Fault Tolerance}. In \bibinfo{booktitle}{\emph{2013 IEEE 33rd International Conference on Distributed Computing Systems}}. \bibinfo{pages}{297--306}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/ICDCS.2013.53}
\showDOI{\tempurl}


\bibitem[Badertscher et~al\mbox{.}(2021)]%
        {Badertscher2021BitcoinRPD51}
\bibfield{author}{\bibinfo{person}{Christian Badertscher}, \bibinfo{person}{Yun Lu}, {and} \bibinfo{person}{Vassilis Zikas}.} \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{A Rational Protocol Treatment of 51{\%} Attacks}. In \bibinfo{booktitle}{\emph{Advances in Cryptology -- CRYPTO 2021}}, \bibfield{editor}{\bibinfo{person}{Tal Malkin} {and} \bibinfo{person}{Chris Peikert}} (Eds.). \bibinfo{publisher}{Springer International Publishing}, \bibinfo{address}{Cham}, \bibinfo{pages}{3--32}.
\newblock
\showISBNx{978-3-030-84252-9}


\bibitem[Blum et~al\mbox{.}(2021)]%
        {blum2021tardigrade}
\bibfield{author}{\bibinfo{person}{Erica Blum}, \bibinfo{person}{Jonathan Katz}, {and} \bibinfo{person}{Julian Loss}.} \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{Tardigrade: An atomic broadcast protocol for arbitrary network conditions}. In \bibinfo{booktitle}{\emph{Advances in Cryptology--ASIACRYPT 2021: 27th International Conference on the Theory and Application of Cryptology and Information Security, Singapore, December 6--10, 2021, Proceedings, Part II 27}}. Springer, \bibinfo{pages}{547--572}.
\newblock


\bibitem[Bracha(1987)]%
        {Bracha1987AsyncBFT}
\bibfield{author}{\bibinfo{person}{Gabriel Bracha}.} \bibinfo{year}{1987}\natexlab{}.
\newblock \showarticletitle{Asynchronous Byzantine agreement protocols}.
\newblock \bibinfo{journal}{\emph{Information and Computation}} \bibinfo{volume}{75}, \bibinfo{number}{2} (\bibinfo{year}{1987}), \bibinfo{pages}{130--143}.
\newblock
\showISSN{0890-5401}
\urldef\tempurl%
\url{https://doi.org/10.1016/0890-5401(87)90054-X}
\showDOI{\tempurl}


\bibitem[Cachin et~al\mbox{.}(2001)]%
        {Cachin2001AsyncBroadcast}
\bibfield{author}{\bibinfo{person}{Christian Cachin}, \bibinfo{person}{Klaus Kursawe}, \bibinfo{person}{Frank Petzold}, {and} \bibinfo{person}{Victor Shoup}.} \bibinfo{year}{2001}\natexlab{}.
\newblock \bibinfo{title}{Secure and Efficient Asynchronous Broadcast Protocols}.
\newblock
\newblock
\showISBNx{978-3-540-42456-7}
\urldef\tempurl%
\url{https://doi.org/10.1007/3-540-44647-8_31}
\showDOI{\tempurl}


\bibitem[Cachin et~al\mbox{.}(2000)]%
        {Cachin2000AsyncAgreement}
\bibfield{author}{\bibinfo{person}{Christian Cachin}, \bibinfo{person}{Klaus Kursawe}, {and} \bibinfo{person}{Victor Shoup}.} \bibinfo{year}{2000}\natexlab{}.
\newblock \showarticletitle{Random Oracles in Constantipole: Practical Asynchronous Byzantine Agreement Using Cryptography}. In \bibinfo{booktitle}{\emph{Proceedings of the Nineteenth Annual ACM Symposium on Principles of Distributed Computing (PODC)}} (Portland, Oregon, USA) \emph{(\bibinfo{series}{PODC '00})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{123–132}.
\newblock
\showISBNx{1581131836}
\urldef\tempurl%
\url{https://doi.org/10.1145/343477.343531}
\showDOI{\tempurl}


\bibitem[Castro and Liskov(1999)]%
        {CastroLiskov1999pBFT}
\bibfield{author}{\bibinfo{person}{Miguel Castro} {and} \bibinfo{person}{Barbara Liskov}.} \bibinfo{year}{1999}\natexlab{}.
\newblock \showarticletitle{Practical Byzantine Fault Tolerance}. In \bibinfo{booktitle}{\emph{Proceedings of the Third Symposium on Operating Systems Design and Implementation}} (New Orleans, Louisiana, USA) \emph{(\bibinfo{series}{OSDI '99})}. \bibinfo{publisher}{USENIX Association}, \bibinfo{address}{USA}, \bibinfo{pages}{173–186}.
\newblock
\showISBNx{1880446391}


\bibitem[Chen et~al\mbox{.}(2022)]%
        {Chen2022SNARKS}
\bibfield{author}{\bibinfo{person}{Megan Chen}, \bibinfo{person}{Alessandro Chiesa}, {and} \bibinfo{person}{Nicholas Spooner}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{On Succinct Non-Interactive Arguments In Relativized Worlds}. In \bibinfo{booktitle}{\emph{Advances in Cryptology – EUROCRYPT 2022: 41st Annual International Conference on the Theory and Applications of Cryptographic Techniques, Trondheim, Norway, May 30 – June 3, 2022, Proceedings, Part II}} (Trondheim, Norway). \bibinfo{publisher}{Springer-Verlag}, \bibinfo{address}{Berlin, Heidelberg}, \bibinfo{pages}{336–366}.
\newblock
\showISBNx{978-3-031-07084-6}
\urldef\tempurl%
\url{https://doi.org/10.1007/978-3-031-07085-3_12}
\showDOI{\tempurl}


\bibitem[Civit et~al\mbox{.}(2021)]%
        {Civit2021Polygraph}
\bibfield{author}{\bibinfo{person}{Pierre Civit}, \bibinfo{person}{Seth Gilbert}, {and} \bibinfo{person}{Vincent Gramoli}.} \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{Polygraph: Accountable Byzantine Agreement}. In \bibinfo{booktitle}{\emph{2021 IEEE 41st International Conference on Distributed Computing Systems (ICDCS)}}. \bibinfo{pages}{403--413}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/ICDCS51616.2021.00046}
\showDOI{\tempurl}


\bibitem[Cristian et~al\mbox{.}(1995)]%
        {Cristian1995ATOMICBF}
\bibfield{author}{\bibinfo{person}{Flaviu Cristian}, \bibinfo{person}{Houtan Aghili}, \bibinfo{person}{H.~Raymond Strong}, {and} \bibinfo{person}{Danny Dolev}.} \bibinfo{year}{1995}\natexlab{}.
\newblock \showarticletitle{ATOMIC BROADCAST: FROM SIMPLE MESSAGE DIFFUSION TO BYZANTINE AGREEMENT}.
\newblock \bibinfo{journal}{\emph{Twenty-Fifth International Symposium on Fault-Tolerant Computing, 1995, ' Highlights from Twenty-Five Years'.}} (\bibinfo{year}{1995}), \bibinfo{pages}{431--}.
\newblock


\bibitem[Dolev and Strong(1983)]%
        {Dolev1983AuthenticatedByzantine}
\bibfield{author}{\bibinfo{person}{D. Dolev} {and} \bibinfo{person}{H.~R. Strong}.} \bibinfo{year}{1983}\natexlab{}.
\newblock \showarticletitle{Authenticated Algorithms for Byzantine Agreement}.
\newblock \bibinfo{journal}{\emph{SIAM J. Comput.}} \bibinfo{volume}{12}, \bibinfo{number}{4} (\bibinfo{date}{nov} \bibinfo{year}{1983}), \bibinfo{pages}{656–666}.
\newblock
\showISSN{0097-5397}
\urldef\tempurl%
\url{https://doi.org/10.1137/0212045}
\showDOI{\tempurl}


\bibitem[Dwork et~al\mbox{.}(1988)]%
        {Cynthia1988PartialSynchrony}
\bibfield{author}{\bibinfo{person}{Cynthia Dwork}, \bibinfo{person}{Nancy Lynch}, {and} \bibinfo{person}{Larry Stockmeyer}.} \bibinfo{year}{1988}\natexlab{}.
\newblock \showarticletitle{Consensus in the Presence of Partial Synchrony}.
\newblock \bibinfo{journal}{\emph{J. ACM}} \bibinfo{volume}{35}, \bibinfo{number}{2} (\bibinfo{date}{apr} \bibinfo{year}{1988}), \bibinfo{pages}{288–323}.
\newblock
\showISSN{0004-5411}
\urldef\tempurl%
\url{https://doi.org/10.1145/42282.42283}
\showDOI{\tempurl}


\bibitem[Ephraim et~al\mbox{.}(2020)]%
        {Ephraim2020SPARK}
\bibfield{author}{\bibinfo{person}{Naomi Ephraim}, \bibinfo{person}{Cody Freitag}, \bibinfo{person}{Ilan Komargodski}, {and} \bibinfo{person}{Rafael Pass}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{SPARKs: Succinct Parallelizable Arguments of Knowledge}. In \bibinfo{booktitle}{\emph{Advances in Cryptology -- EUROCRYPT 2020}}, \bibfield{editor}{\bibinfo{person}{Anne Canteaut} {and} \bibinfo{person}{Yuval Ishai}} (Eds.). \bibinfo{publisher}{Springer International Publishing}, \bibinfo{address}{Cham}, \bibinfo{pages}{707--737}.
\newblock
\showISBNx{978-3-030-45721-1}


\bibitem[Fischer et~al\mbox{.}(1985)]%
        {Fischer1985ImpossibilityAsync}
\bibfield{author}{\bibinfo{person}{Michael~J. Fischer}, \bibinfo{person}{Nancy~A. Lynch}, {and} \bibinfo{person}{Michael~S. Paterson}.} \bibinfo{year}{1985}\natexlab{}.
\newblock \showarticletitle{Impossibility of Distributed Consensus with One Faulty Process}.
\newblock \bibinfo{journal}{\emph{J. ACM}} \bibinfo{volume}{32}, \bibinfo{number}{2} (\bibinfo{date}{apr} \bibinfo{year}{1985}), \bibinfo{pages}{374–382}.
\newblock
\showISSN{0004-5411}
\urldef\tempurl%
\url{https://doi.org/10.1145/3149.214121}
\showDOI{\tempurl}


\bibitem[Ganesh et~al\mbox{.}(2022)]%
        {Ganesh2022RationalCrypto}
\bibfield{author}{\bibinfo{person}{Chaya Ganesh}, \bibinfo{person}{Bhavana Kanukurthi}, {and} \bibinfo{person}{Girisha Shankar}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{Secure Auctions in the Presence of Rational Adversaries}. In \bibinfo{booktitle}{\emph{Proceedings of the 2022 ACM SIGSAC Conference on Computer and Communications Security}} (Los Angeles, CA, USA) \emph{(\bibinfo{series}{CCS '22})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{1173–1186}.
\newblock
\showISBNx{9781450394505}
\urldef\tempurl%
\url{https://doi.org/10.1145/3548606.3560706}
\showDOI{\tempurl}


\bibitem[Gao et~al\mbox{.}(2022)]%
        {Gao2022Async2}
\bibfield{author}{\bibinfo{person}{Yingzi Gao}, \bibinfo{person}{Yuan Lu}, \bibinfo{person}{Zhenliang Lu}, \bibinfo{person}{Qiang Tang}, \bibinfo{person}{Jing Xu}, {and} \bibinfo{person}{Zhenfeng Zhang}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{Dumbo-NG: Fast Asynchronous BFT Consensus with Throughput-Oblivious Latency}. In \bibinfo{booktitle}{\emph{Proceedings of the 2022 ACM SIGSAC Conference on Computer and Communications Security}} (Los Angeles, CA, USA) \emph{(\bibinfo{series}{CCS '22})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{1187–1201}.
\newblock
\showISBNx{9781450394505}
\urldef\tempurl%
\url{https://doi.org/10.1145/3548606.3559379}
\showDOI{\tempurl}


\bibitem[Garay et~al\mbox{.}(2015a)]%
        {Garay2015Backbone}
\bibfield{author}{\bibinfo{person}{Juan Garay}, \bibinfo{person}{Aggelos Kiayias}, {and} \bibinfo{person}{Nikos Leonardos}.} \bibinfo{year}{2015}\natexlab{a}.
\newblock \showarticletitle{The Bitcoin Backbone Protocol: Analysis and Applications}. In \bibinfo{booktitle}{\emph{Advances in Cryptology - EUROCRYPT 2015}}, \bibfield{editor}{\bibinfo{person}{Elisabeth Oswald} {and} \bibinfo{person}{Marc Fischlin}} (Eds.). \bibinfo{publisher}{Springer Berlin Heidelberg}, \bibinfo{address}{Berlin, Heidelberg}, \bibinfo{pages}{281--310}.
\newblock
\showISBNx{978-3-662-46803-6}


\bibitem[Garay et~al\mbox{.}(2015b)]%
        {garay2015Bitcoin}
\bibfield{author}{\bibinfo{person}{Juan Garay}, \bibinfo{person}{Aggelos Kiayias}, {and} \bibinfo{person}{Nikos Leonardos}.} \bibinfo{year}{2015}\natexlab{b}.
\newblock \showarticletitle{The Bitcoin Backbone Protocol: Analysis and Applications}.
\newblock \bibinfo{journal}{\emph{Advances in Cryptology-EUROCRYPT 2015}} (\bibinfo{year}{2015}), \bibinfo{pages}{281--310}.
\newblock


\bibitem[Garay et~al\mbox{.}(2013)]%
        {Garay2013RPD}
\bibfield{author}{\bibinfo{person}{Juan~A. Garay}, \bibinfo{person}{Jonathan Katz}, \bibinfo{person}{Ueli Maurer}, \bibinfo{person}{Bj{\"o}rn Tackmann}, {and} \bibinfo{person}{Vassilis Zikas}.} \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{Rational Protocol Design: Cryptography against Incentive-Driven Adversaries}.
\newblock \bibinfo{journal}{\emph{2013 IEEE 54th Annual Symposium on Foundations of Computer Science}} (\bibinfo{year}{2013}), \bibinfo{pages}{648--657}.
\newblock


\bibitem[Gilad et~al\mbox{.}(2017)]%
        {Micali2017Algorand}
\bibfield{author}{\bibinfo{person}{Yossi Gilad}, \bibinfo{person}{Rotem Hemo}, \bibinfo{person}{Silvio Micali}, \bibinfo{person}{Georgios Vlachos}, {and} \bibinfo{person}{Nickolai Zeldovich}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Algorand: Scaling Byzantine Agreements for Cryptocurrencies}. In \bibinfo{booktitle}{\emph{Proceedings of the 26th Symposium on Operating Systems Principles}} (Shanghai, China) \emph{(\bibinfo{series}{SOSP '17})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{51–68}.
\newblock
\showISBNx{9781450350853}
\urldef\tempurl%
\url{https://doi.org/10.1145/3132747.3132757}
\showDOI{\tempurl}


\bibitem[Groce et~al\mbox{.}(2012)]%
        {katz2012RC}
\bibfield{author}{\bibinfo{person}{Adam Groce}, \bibinfo{person}{Jonathan Katz}, \bibinfo{person}{Aishwarya Thiruvengadam}, {and} \bibinfo{person}{Vassilis Zikas}.} \bibinfo{year}{2012}\natexlab{}.
\newblock \showarticletitle{Byzantine Agreement with a Rational Adversary}. In \bibinfo{booktitle}{\emph{Automata, Languages, and Programming}}, \bibfield{editor}{\bibinfo{person}{Artur Czumaj}, \bibinfo{person}{Kurt Mehlhorn}, \bibinfo{person}{Andrew Pitts}, {and} \bibinfo{person}{Roger Wattenhofer}} (Eds.). \bibinfo{publisher}{Springer Berlin Heidelberg}, \bibinfo{address}{Berlin, Heidelberg}, \bibinfo{pages}{561--572}.
\newblock
\showISBNx{978-3-642-31585-5}


\bibitem[Karantias et~al\mbox{.}(2020)]%
        {Kiayias2020PoB}
\bibfield{author}{\bibinfo{person}{Kostis Karantias}, \bibinfo{person}{Aggelos Kiayias}, {and} \bibinfo{person}{Dionysis Zindros}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{Proof-of-Burn}. In \bibinfo{booktitle}{\emph{Financial Cryptography and Data Security: 24th International Conference, FC 2020}} (Kota Kinabalu, Malaysia). \bibinfo{publisher}{Springer-Verlag}, \bibinfo{address}{Berlin, Heidelberg}, \bibinfo{pages}{523–540}.
\newblock
\showISBNx{978-3-030-51279-8}
\urldef\tempurl%
\url{https://doi.org/10.1007/978-3-030-51280-4_28}
\showDOI{\tempurl}


\bibitem[Katz and Koo(2006)]%
        {Katz2006thresholds}
\bibfield{author}{\bibinfo{person}{Jonathan Katz} {and} \bibinfo{person}{Chiu-Yuen Koo}.} \bibinfo{year}{2006}\natexlab{}.
\newblock \showarticletitle{On expected constant-round protocols for Byzantine agreement}. In \bibinfo{booktitle}{\emph{Annual International Cryptology Conference}}. Springer, \bibinfo{pages}{445--462}.
\newblock


\bibitem[Lamport(1998)]%
        {Lamport1998Paxos}
\bibfield{author}{\bibinfo{person}{Leslie Lamport}.} \bibinfo{year}{1998}\natexlab{}.
\newblock \showarticletitle{The Part-Time Parliament}.
\newblock \bibinfo{journal}{\emph{ACM Trans. Comput. Syst.}} \bibinfo{volume}{16}, \bibinfo{number}{2} (\bibinfo{date}{may} \bibinfo{year}{1998}), \bibinfo{pages}{133–169}.
\newblock
\showISSN{0734-2071}
\urldef\tempurl%
\url{https://doi.org/10.1145/279227.279229}
\showDOI{\tempurl}


\bibitem[Lamport(2001)]%
        {Lamport2001Paxos}
\bibfield{author}{\bibinfo{person}{Leslie Lamport}.} \bibinfo{year}{2001}\natexlab{}.
\newblock \showarticletitle{Paxos Made Simple}.
\newblock \bibinfo{journal}{\emph{ACM SIGACT News (Distributed Computing Column) 32, 4 (Whole Number 121, December 2001)}} (\bibinfo{date}{December} \bibinfo{year}{2001}), \bibinfo{pages}{51--58}.
\newblock
\urldef\tempurl%
\url{https://www.microsoft.com/en-us/research/publication/paxos-made-simple/}
\showURL{%
\tempurl}


\bibitem[Lamport et~al\mbox{.}(1982a)]%
        {Lamport1982BGP}
\bibfield{author}{\bibinfo{person}{Leslie Lamport}, \bibinfo{person}{Robert Shostak}, {and} \bibinfo{person}{Marshall Pease}.} \bibinfo{year}{1982}\natexlab{a}.
\newblock \showarticletitle{The Byzantine Generals Problem}.
\newblock \bibinfo{journal}{\emph{ACM Trans. Program. Lang. Syst.}} \bibinfo{volume}{4}, \bibinfo{number}{3} (\bibinfo{date}{jul} \bibinfo{year}{1982}), \bibinfo{pages}{382–401}.
\newblock
\showISSN{0164-0925}
\urldef\tempurl%
\url{https://doi.org/10.1145/357172.357176}
\showDOI{\tempurl}


\bibitem[Lamport et~al\mbox{.}(1982b)]%
        {LSP1982}
\bibfield{author}{\bibinfo{person}{Leslie Lamport}, \bibinfo{person}{Robert Shostak}, {and} \bibinfo{person}{Marshall Pease}.} \bibinfo{year}{1982}\natexlab{b}.
\newblock \showarticletitle{The Byzantine Generals Problem}.
\newblock \bibinfo{journal}{\emph{ACM Trans. Program. Lang. Syst.}} \bibinfo{volume}{4}, \bibinfo{number}{3} (\bibinfo{date}{jul} \bibinfo{year}{1982}), \bibinfo{pages}{382–401}.
\newblock
\showISSN{0164-0925}
\urldef\tempurl%
\url{https://doi.org/10.1145/357172.357176}
\showDOI{\tempurl}


\bibitem[Lu et~al\mbox{.}(2022)]%
        {Lu2022Async4}
\bibfield{author}{\bibinfo{person}{Yuan Lu}, \bibinfo{person}{Zhenliang Lu}, {and} \bibinfo{person}{Qiang Tang}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{Bolt-Dumbo Transformer: Asynchronous Consensus As Fast As the Pipelined BFT}. In \bibinfo{booktitle}{\emph{Proceedings of the 2022 ACM SIGSAC Conference on Computer and Communications Security}} (Los Angeles, CA, USA) \emph{(\bibinfo{series}{CCS '22})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{2159–2173}.
\newblock
\showISBNx{9781450394505}
\urldef\tempurl%
\url{https://doi.org/10.1145/3548606.3559346}
\showDOI{\tempurl}


\bibitem[Malkhi et~al\mbox{.}(2019)]%
        {Malkhi2019FlexibleBFT}
\bibfield{author}{\bibinfo{person}{Dahlia Malkhi}, \bibinfo{person}{Kartik Nayak}, {and} \bibinfo{person}{Ling Ren}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Flexible Byzantine Fault Tolerance}. In \bibinfo{booktitle}{\emph{Proceedings of the 2019 ACM SIGSAC Conference on Computer and Communications Security}} (London, United Kingdom) \emph{(\bibinfo{series}{CCS '19})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{1041–1053}.
\newblock
\showISBNx{9781450367479}
\urldef\tempurl%
\url{https://doi.org/10.1145/3319535.3354225}
\showDOI{\tempurl}


\bibitem[Miller et~al\mbox{.}(2016)]%
        {Miller2016Honeybadger}
\bibfield{author}{\bibinfo{person}{Andrew Miller}, \bibinfo{person}{Yu Xia}, \bibinfo{person}{Kyle Croman}, \bibinfo{person}{Elaine Shi}, {and} \bibinfo{person}{Dawn Song}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{The Honey Badger of BFT Protocols}. In \bibinfo{booktitle}{\emph{Proceedings of the 2016 ACM SIGSAC Conference on Computer and Communications Security}} (Vienna, Austria) \emph{(\bibinfo{series}{CCS '16})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{31–42}.
\newblock
\showISBNx{9781450341394}
\urldef\tempurl%
\url{https://doi.org/10.1145/2976749.2978399}
\showDOI{\tempurl}


\bibitem[Nakamoto(2009)]%
        {nakamoto2009Bitcoin}
\bibfield{author}{\bibinfo{person}{Satoshi Nakamoto}.} \bibinfo{year}{2009}\natexlab{}.
\newblock \bibinfo{title}{Bitcoin : A Peer-to-Peer Electronic Cash System}.
\newblock
\newblock


\bibitem[Ongaro and Ousterhout(2014)]%
        {Ongaro2014Raft}
\bibfield{author}{\bibinfo{person}{Diego Ongaro} {and} \bibinfo{person}{John Ousterhout}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{In Search of an Understandable Consensus Algorithm}. In \bibinfo{booktitle}{\emph{Proceedings of the 2014 USENIX Conference on USENIX Annual Technical Conference}} (Philadelphia, PA) \emph{(\bibinfo{series}{USENIX ATC'14})}. \bibinfo{publisher}{USENIX Association}, \bibinfo{address}{USA}, \bibinfo{pages}{305–320}.
\newblock
\showISBNx{9781931971102}


\bibitem[Pease et~al\mbox{.}(1980)]%
        {Pease1980LSPInception}
\bibfield{author}{\bibinfo{person}{M. Pease}, \bibinfo{person}{R. Shostak}, {and} \bibinfo{person}{L. Lamport}.} \bibinfo{year}{1980}\natexlab{}.
\newblock \showarticletitle{Reaching Agreement in the Presence of Faults}.
\newblock \bibinfo{journal}{\emph{J. ACM}} \bibinfo{volume}{27}, \bibinfo{number}{2} (\bibinfo{date}{apr} \bibinfo{year}{1980}), \bibinfo{pages}{228–234}.
\newblock
\showISSN{0004-5411}
\urldef\tempurl%
\url{https://doi.org/10.1145/322186.322188}
\showDOI{\tempurl}


\bibitem[Ranchal-Pedrosa and Gramoli(2020)]%
        {Ranchal2020ZLBAccountable}
\bibfield{author}{\bibinfo{person}{Alejandro Ranchal-Pedrosa} {and} \bibinfo{person}{Vincent Gramoli}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{ZLB: A blockchain to tolerate colluding majorities}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2007.10541}} (\bibinfo{year}{2020}).
\newblock


\bibitem[Ranchal-Pedrosa and Gramoli(2022)]%
        {Gramoli2022Trap}
\bibfield{author}{\bibinfo{person}{Alejandro Ranchal-Pedrosa} {and} \bibinfo{person}{Vincent Gramoli}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{TRAP: The Bait of Rational Players to Solve Byzantine Consensus}. In \bibinfo{booktitle}{\emph{Proceedings of the 2022 ACM on Asia Conference on Computer and Communications Security}} (Nagasaki, Japan) \emph{(\bibinfo{series}{ASIA CCS '22})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{168–181}.
\newblock
\showISBNx{9781450391405}
\urldef\tempurl%
\url{https://doi.org/10.1145/3488932.3517386}
\showDOI{\tempurl}


\bibitem[Schelling(1963)]%
        {Schelling1963SoC}
\bibfield{author}{\bibinfo{person}{Thomas~C. Schelling}.} \bibinfo{year}{1963}\natexlab{}.
\newblock \bibinfo{booktitle}{\emph{The strategy of Conflict}}.
\newblock \bibinfo{publisher}{Oxford University Press}.
\newblock


\bibitem[Spiegelman et~al\mbox{.}(2022)]%
        {Spiegelman2022Async3}
\bibfield{author}{\bibinfo{person}{Alexander Spiegelman}, \bibinfo{person}{Neil Giridharan}, \bibinfo{person}{Alberto Sonnino}, {and} \bibinfo{person}{Lefteris Kokoris-Kogias}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{Bullshark: DAG BFT Protocols Made Practical}. In \bibinfo{booktitle}{\emph{Proceedings of the 2022 ACM SIGSAC Conference on Computer and Communications Security}} (Los Angeles, CA, USA) \emph{(\bibinfo{series}{CCS '22})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{2705–2718}.
\newblock
\showISBNx{9781450394505}
\urldef\tempurl%
\url{https://doi.org/10.1145/3548606.3559361}
\showDOI{\tempurl}


\bibitem[Vila{\c{c}}a et~al\mbox{.}(2011)]%
        {Fernandez2011BARPODS}
\bibfield{author}{\bibinfo{person}{Xavier Vila{\c{c}}a}, \bibinfo{person}{Jo{\~a}o Leit{\~a}o}, \bibinfo{person}{Miguel Correia}, {and} \bibinfo{person}{Lu{\'i}s Rodrigues}.} \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{N-party BAR Transfer}. In \bibinfo{booktitle}{\emph{Principles of Distributed Systems}}, \bibfield{editor}{\bibinfo{person}{Antonio Fern{\`a}ndez~Anta}, \bibinfo{person}{Giuseppe Lipari}, {and} \bibinfo{person}{Matthieu Roy}} (Eds.). \bibinfo{publisher}{Springer Berlin Heidelberg}, \bibinfo{address}{Berlin, Heidelberg}, \bibinfo{pages}{392--408}.
\newblock
\showISBNx{978-3-642-25873-2}


\bibitem[Vila\c{c}a et~al\mbox{.}(2011)]%
        {Vilacca2011BARIntro}
\bibfield{author}{\bibinfo{person}{Xavier Vila\c{c}a}, \bibinfo{person}{Jo\~{a}o Leit\~{a}o}, {and} \bibinfo{person}{Lu\'{\i}s Rodrigues}.} \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{N-Party BAR Transfer: Motivation, Definition, and Challenges}. In \bibinfo{booktitle}{\emph{Proceedings of the 3rd International Workshop on Theoretical Aspects of Dynamic Distributed Systems}} (Rome, Italy) \emph{(\bibinfo{series}{TADDS '11})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{18–22}.
\newblock
\showISBNx{9781450309462}
\urldef\tempurl%
\url{https://doi.org/10.1145/2034640.2034647}
\showDOI{\tempurl}


\bibitem[Yin et~al\mbox{.}(2019)]%
        {Yin2019Hotstuff}
\bibfield{author}{\bibinfo{person}{Maofan Yin}, \bibinfo{person}{Dahlia Malkhi}, \bibinfo{person}{Michael~K. Reiter}, \bibinfo{person}{Guy~Golan Gueta}, {and} \bibinfo{person}{Ittai Abraham}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{HotStuff: BFT Consensus with Linearity and Responsiveness}. In \bibinfo{booktitle}{\emph{Proceedings of the 2019 ACM Symposium on Principles of Distributed Computing}} (Toronto ON, Canada) \emph{(\bibinfo{series}{PODC '19})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{347–356}.
\newblock
\showISBNx{9781450362177}
\urldef\tempurl%
\url{https://doi.org/10.1145/3293611.3331591}
\showDOI{\tempurl}


\bibitem[Zhang and Duan(2022)]%
        {zhang2022Async1}
\bibfield{author}{\bibinfo{person}{Haibin Zhang} {and} \bibinfo{person}{Sisi Duan}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{PACE: Fully Parallelizable BFT from Reproposable Byzantine Agreement}. In \bibinfo{booktitle}{\emph{Proceedings of the 2022 ACM SIGSAC Conference on Computer and Communications Security}} (Los Angeles, CA, USA) \emph{(\bibinfo{series}{CCS '22})}. \bibinfo{publisher}{Association for Computing Machinery}, \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{3151–3164}.
\newblock
\showISBNx{9781450394505}
\urldef\tempurl%
\url{https://doi.org/10.1145/3548606.3559348}
\showDOI{\tempurl}


\end{thebibliography}

